Language Models are Causal Knowledge Extractors for Zero-shot Video Question Answering

Causal Video Question Answering (CVidQA) queries not only association or temporal relations but also causal relations in a video. Existing question synthesis methods pre-trained question generation (QG) systems on reading comprehension datasets with text descriptions as inputs. However, QG models only learn to ask association questions (e.g., ``what is someone doing...'') and result in inferior performance due to the poor transfer of association knowledge to CVidQA, which focuses on causal questions like ``why is someone doing ...''. Observing this, we proposed to exploit causal knowledge to generate question-answer pairs, and proposed a novel framework, Causal Knowledge Extraction from Language Models (CaKE-LM), leveraging causal commonsense knowledge from language models to tackle CVidQA. To extract knowledge from LMs, CaKE-LM generates causal questions containing two events with one triggering another (e.g., ``score a goal'' triggers ``soccer player kicking ball'') by prompting LM with the action (soccer player kicking ball) to retrieve the intention (to score a goal). CaKE-LM significantly outperforms conventional methods by 4% to 6% of zero-shot CVidQA accuracy on NExT-QA and Causal-VidQA datasets. We also conduct comprehensive analyses and provide key findings for future research.

==> figures/lm_dist.tex <==
\begin{figure*}[!ht]
\centering
\includegraphics[width=\linewidth]{figures/lm_dist_img.pdf}
\caption{\textbf{Cumulative distribution of LM response lengths that reflects LM response quality.} X axis represents the token length of response and Y axis shows the ratio of the dataset. (Section \ref{subsec:LM_ana}) }
\label{lm_dist}
\end{figure*}

==> section/1-intro-old.tex <==
\section{Introduction}
Video Question Answering (VidQA), which queries a video clip with a natural language question, is a crucial task in natural language processing and computer vision. Recent studies move a step forward to \task{} (\taskabbr{}) where the questions are about \textbf{causal relations} of actions and events. For example, \textit{Why is the man in the video running} is a causal question that queries an event not only \textit{before}, but also the \textit{intention} of the man running. This setting is more challenging because the model needs to not only discover the associated actions or events in a video but also figure out the causal relations between them. Modern \taskabbr{} systems \cite{model_2.5+1D,model_xiao2021hgqa,model_xiao2022vgt} decoupled video into object-level and developed graph reasoning networks to obtain fine-grained representation of videos and reached significant performance on \taskabbr{} dataset, NExT-QA \cite{dataset_xiao2021nextqa}. However, these supervised methods relied on massive question-answer pairs to learn the mapping between videos, inquired events, and causal relations, but a single dataset can hardly cover all scenarios in the ever-changing world. 
%===Need example?
Furthermore, recollecting a dataset for every new application is costly and unscalable.
%assumed there always existed large-scale datasets to learn the mapping from video-questions to answers, but 
%different applications 
%practically it is costly and unscalable to collect \taskabbr{} data for ever-changing world with different sources, activities, actions or objects for developing applications. 
Therefore, dataset allocation becomes a critical issue to leverage state-of-the-art \taskabbr{} systems in practice.
%===also argue dataset's domain is narrow?

%without relying on a specific, explicit human annotation as a knowledge source,
To develop a \taskabbr{} data allocation solution that is quickly adaptable and scalable to new environments,  we argue several prerequisites to acquire causal knowledge: The knowledge source should (1) cover broad domains instead of a specific one. (2) be implicitly learned rather than explicitly fitting human-defined patterns. Traditional VidQA tackled this problem by utilizing text question generation systems \cite{heilman2009question,T5_JMLR:v21:20-074} to automatically label training question-answers according to video descriptions \cite{videoqaaaai2017,xu2017msvdqavideo,yang2021justask,yang2022justaskplus}. 
%name this paradigm? cite GPN?
Nevertheless, this paradigm strongly relied on pre-defined templates \cite{videoqaaaai2017,xu2017msvdqavideo} or pre-training datasets \cite{yang2021justask,yang2022justaskplus}.  For example, the state-of-the-art approach in this category \cite{yang2021justask}, leveraged \textit{factoid} QA dataset SQuAD \cite{rajpurkar-etal-2016-squad} pre-trained question generator. However, relying on specific datasets as explicit knowledge sources results in poor adaptability and scalability to new applications. Therefore, while \cite{yang2021justask} obtained knowledge from a large-scale, human-labeled dataset, it performed sub-optimal on \textit{causal} questions in particular (6\% worse compared to overall performance).
%define descriptive 

%To develop a general \taskabbr{} solution that is quickly adaptable and scalable to new environments without relying on a specific, explicit human annotation as a knowledge source, we argue several prerequisites to acquire causal knowledge: The knowledge should (1) cover broad domains instead of a specific one. (2) be implicitly learned rather than explicitly fitting human-defined patterns. (3) training with no or few human annotations required. (4) extractable without or with few re-training or data allocation. 

Observing this, we propose a novel framework, \textbf{\ours{} (\oursabbr{})}, leveraging Language Models (LMs) knowledge to tackle challenging \taskabbr{} tasks. LMs can be trained with massive data crossing various sources such as Wikipedia, news, forums, books, or dialogues in a implicit and self-supervised manner without relying on a specific human annotated patterns. Recent literature also suggested that LMs learns causal knowledge from pre-training and can be utilized in understanding chat-bot user intentions with dialogues \cite{lmappint1_sahu-etal-2022-data,lmappint2_rosenbaum-etal-2022-linguist,lmappint3_zhang-etal-2022-fine} or classify cause-effect relations \cite{lmappce1_hosseini-etal-2022-knowledge}.

%To extract knowledge, \oursabbr{} prompts the LM with video descriptions and generate QAs for \taskabbr{} training. 
Recent studies \cite{lm_gui2021kat,lm_pica_yang2021empirical} revealed that in-context learning is capable to extract knowledge from LM to tackle knowledge visual QA tasks. Different from previous work that utilize LM as a knowledge base for \textit{factoid} QAs, we move a step further to extract \textit{causal} knowledge from LMs to estimate the intention of actions or events. Specifically, \oursabbr{} prompts the LM with video descriptions and generate QAs for \taskabbr{} training. We also investigate how the scale of LM and example size of in-context effect the performance, causal knowledge distillability from a LM to another one, and the information gap between text descriptions and videos.
%in context learning
%Different from previous

%1. knowledge 2. learning/patterns 3. extraction

%Observing the success of language models (LMs) in knowledge VQA \cite{lm_gui2021kat,lm_pica_yang2021empirical} and representation learning \cite{lm_zhao2022lavila}, we propose \ours{} (\oursabbr{}), explore the opportunity of leveraging LMs for \taskabbr{} to demonstrate and investigate the potential of LMs in challenging visual reasoning tasks. Specifically, we prompt LMs with captions for intentions of actions or events, and convert captions and LM responses to QAS to train video QA models. To alleviate the visual mis-aligned responses due to captioning information loss, we develop a \ourscomp{} (\ourscompabbr{}) that estimates the matching score between the video and LM responses. Compared to conventional approaches, our method extracts LM knowledge by prompting and therefore is controllable and scalable. In addition, our method does not require further training resources, explicit knowledge, or annotation efforts. 

%knowledge come from many domains, not a specific
%conditions: 1. implicit 2, general 3. no annotation
%we seek an alternative approach:
%As web collected  
%explain why ja worked for traditional but not causal ones
%domain gaps between NLP datasets and visual descriptions
%mapping from passage to qas



%Recently, \task{} (\taskabbr) has attracted both computer vision and natural language processing communities. Compared to traditional Video QA tasks , \taskabbr{} \cite{dataset_li2022causalvidqa,dataset_xiao2021nextqa} is more challenging because the model needs to comprehend not only surface signals such as objects, actions, and their spatial or temporal relations, but also causal relations between actions or events. While there is a significant process \cite{model_2.5+1D,model_xiao2021hgqa,model_xiao2022vgt} thanks to modern deep learning models and large-scale datasets, the annotation cost remains a burden for the development of \taskabbr{} systems.

\input{figures/motivation.tex}


Experimental results demonstrates 10\% to 32\% of accuracy improvement on causal questions on two large-scale \taskabbr{} datasets, NExT-QA \cite{dataset_xiao2021nextqa} and Causal-VidQA \cite{dataset_li2022causalvidqa}. On Causal-VidQA benchmark, \oursabbr{} even outperforms supervised methods without using any human labeled video-question-answer triples. We also explore several key findings: (1) Causal knowledge in LMs can be extracted for video reasoning tasks by caption prompting, without fine-tuning or few-shot learning. (2) Causal knowledge can be distilled from large LMs to smaller ones by training with LM responses. (3) Regardless of significantly fewer parameters, smaller LMs (GPT-Neo 1.3B/2.7B) can reach performance comparable to GPT-3 (<1.0\% accuracy gap), revealing a promising direction of extracting knowledge from LMs for other visual reasoning tasks. (4) Despite the remarkable performance, there are rooms for improvement such as tackling noise and information loss when captioning a video. These experimental results and findings suggest a novel perspective for leveraging LMs for visual reasoning tasks.



%Furthermore, we find that the computation cost of language model inference could be excessive with massive data inputs. Therefore, we present a \oursx{} (\oursxabbr{}), extracting the domain-specific knowledge from a vast and general-purpose language model to a much smaller one. Specifically, we inference a general-purpose language model with small amounts of inputs and train another smaller language model with language model estimated outputs. Doing this allowed us to massively infer LMs without massive computation costs.

%Experimental results demonstrates a huge improvement . We are optimistic that

%setup a new usage of LM?potential on other tasks?

==> section/6-limitations.tex <==
\section{Limitations and Potential Extensions}
%


==> section/7-potential_risks.tex <==
\section{Potential Risks}
As LM knowledge heavily relies on pre-training data, our method may teach \taskabbr{} several biases from language models. For example, gender bias which associate men and women to certain professions or preferences. Future work should to be aware of this and is encouraged to mitigate it in order to develop fair and robust applications.

==> section/_motivation.tex <==
\begin{table}[ht]
\centering
\noindent
\begin{tabular}{|c|c|}
\toprule
 Conventional & Ours \\
Supervised & Unsupervised \\
Explicit & Implicit \\
Specific & General \\


\bottomrule
\end{tabular}

\caption{Motivation}
\label{tab:motivation}
\end{table}

==> tables/freq_words.tex <==
\begin{table*}[ht]
\centering
\noindent
\begin{tabular}{c|c|c|c|c}
& GPT-2 & GPT-Neo (1.3B) & GPT-Neo (2.7B) & GPT-3 \\
\toprule 
\multirow{4}*{0 Shot} 
 & one think like & think like question & think  \textcolor{red}{man} like & entertain fun show \\
 & \textcolor{red}{people}  \textcolor{red}{man} could & know mean  \textcolor{red}{video}  & question mean one & entertainment creating \\
 & know question idea & \textcolor{red}{people} \textcolor{red}{game} one & say know \textcolor{red}{people} &  \textcolor{red}{man} inform viewers \\
 & make \textcolor{red}{game} well  &  \textcolor{red}{man} see \textcolor{red}{two} & \textcolor{red}{two} sentence  \textcolor{red}{video}  & promote joy create \textcolor{red}{game} \\ 
% &  &  &  & \\ 
\midrule
\multirow{4}*{1 Shot}  
 &  \textcolor{red}{man} girl output,&  \textcolor{red}{man}  \textcolor{red}{video} baby   &  \textcolor{red}{man} \textcolor{red}{woman} \textcolor{red}{boy} &  \textcolor{blue}{playing} \textcolor{blue}{singing} music \\
 &  \textcolor{red}{video}  \textcolor{blue}{playing} one & \textcolor{red}{boy} \textcolor{red}{game} girl & baby girl  \textcolor{red}{video}  & \textcolor{red}{game} ask show  \\
 & baby get \textcolor{red}{boy} & play \textcolor{red}{woman}  \textcolor{blue}{playing} & one  \textcolor{blue}{talking}  \textcolor{blue}{playing} & fun making laughing  \\
 & \textcolor{red}{woman} \textcolor{red}{two} like  & get person want & \textcolor{red}{game} person  \textcolor{red}{cartoon} & make take stroller\\ 
% &  &  &  & \\ 
\midrule
\multirow{4}*{5 Shot}  
 &  \textcolor{red}{man} girl one &  \textcolor{red}{man} play  \textcolor{red}{video} &  \textcolor{red}{man}  \textcolor{blue}{playing} play & \textcolor{blue}{singing}  \textcolor{blue}{playing} making \\
 &  \textcolor{red}{video} \textcolor{red}{boy}  \textcolor{blue}{playing} &  \textcolor{blue}{playing} \textcolor{red}{game} baby & \textcolor{red}{game} baby  \textcolor{blue}{talking}  & music showing enjoying \\
 & \textcolor{red}{woman} baby get & \textcolor{red}{boy} get dance  &  \textcolor{red}{video} \textcolor{red}{woman} song  & fun dancing show  \\
 & looking holding guy  & \textcolor{red}{woman} show girl & one car get &  \textcolor{red}{game} laughing stroller\\ 
% &  &  &  & \\ 
%& SL 100\%  & 44.42 & 44.01 & 45.61 & 46.93 & -2.51  \\
\midrule
\multicolumn{5}{c}{Inputs: \textcolor{red}{man}  \textcolor{red}{video}  \textcolor{red}{cartoon}  \textcolor{blue}{talking}  \textcolor{blue}{playing} \textcolor{red}{game} \textcolor{red}{woman} \textcolor{red}{two} \textcolor{red}{people} \textcolor{blue}{singing} \textcolor{red}{boy} \textcolor{red}{stage} } \\
%\midrule
%\multicolumn{5}{c}{man  \textcolor{red}{video}  \textcolor{red}{cartoon}  \textcolor{blue}{talking}  \textcolor{blue}{playing} \textcolor{red}{game} \textcolor{red}{woman} \textcolor{red}{two} \textcolor{red}{people} \textcolor{blue}{singing} \textcolor{red}{boy} stage} \\
\bottomrule
\end{tabular}

\caption{
\textbf{Top 12 generated word of each LM that reveals the LM generation tendency.} 
The bottom row shows top 15 words in input captions. (Section \ref{subsec:LM_ana})
}
\label{tab:freq_words}
\end{table*}
